A determinant approach for generalized $q$-Bernoulli polynomials and asymptotic results

In earlier work, we introduced three families of polynomials where the generating function of each set includes one of the three Jackson $q$-analogs of the Bessel function. This paper gives determinant representation for each family, their large $n $ asymptotics, and two expansion theorems for specific classes of entire functions. We include two examples.

==> bib22.tex <==
% ------------------------------------------------------------------------
% SAMPLE BIBLIOGRAPHY FILE
% ------------------------------------------------------------------------


% ------------------------------------------------------------------------



 %\begin{thebibliography}{10}

@book{ismail,
author={M. E. H.~ Ismail},
title={  {Classical} and {Quantum} Orthogonal {Polynomials} in {One}{ Variable}},
publisher={ Cambridge University Press},
year={ 2005},
address={ Cambridge},
series={Encyclopedia of Mathematics and its Applications},
}



@book{boass,
author={R. P. Boas and R. C. Buck},
title={ {Polynomial} expansions and analytic functions  },
publisher={ Springer-Verlag, Berlin, Heidelberg, New York},
year={ 1958},
}


@book{boass1,
author={R. P. Boas and R. C. Buck},
title={Entire functions  },
publisher={ Academic press, New York},
year={ 1954},
}

@ARTICLE{modified,
author={M.A. Olshanetsky and V.B.K. Rogov},
title={The modified $q$-{Bessel} and the {Bessel}-{Macdonald}{ Functions}
},
journal={arxiv:$q$-alg/9509013. },
volume={},
pages{},
year={1995},}

@ARTICLE{ramis,
author={J. P. Ramis},
title={About the growth of entire functions solutions of linear algebraic
$q$-difference equations},
journal={Ann. Fac. Sci. Toulouse Math. },
volume={1(16)},
pages={53--94},
year={1992},}

@ARTICLE{nac,
author={L. Nachbin},
title={An extension of the notion of integral functions of finite exponential type},
journal={ An. Acad. Brasil. Cienc.},
volume={16},
pages={143--147},
year={1944},}
@Book{Annaby,
author={M. H.~ Annaby and Z. S.~ Mansour},
title={ $q$-Fractional {Calculus} and {Equations}},
series={ Lecture Notes in Mathematics  2056},
publisher={Springer-Verlag.},
address={ Berlin},
year={ 2012},}


@ARTICLE{Cardoss,
author={J. L. ~Cardoso},
title={Basic {Fourier} series convergence on and outside the $q$-{Linear} grid},
journal={J. Fourier Anal. Appl. },
volume={17(1)},
pages={96--114},
year={2011},}

@ARTICLE{Hahn1,
author={H. T. ~Koelink and R. F. Swarttouw},
title={On the zeros of the {Hahn-Exton} $q$-{Bessel} function and associated   $q$-{Lommel} polynomials},
journal={J. Math.  Anal. Appl. },
volume={186},
pages={690--710},
year={1994},}
@ARTICLE{Jackson2,
author={F. H. ~Jackson},
title={A basic-sine and cosine with with symbolical solutions of certain differential equations },
journal={Proc. Edinb. Math. Soc.},
volume={22},
pages={28--38},
year={1903/1904},}
@ARTICLE{Jackson1,
author={F. H. ~Jackson},
title={On $q$-functions and certain difference operator},
journal={Trans. Roy. Soc. Edinb.},
volume={46},
pages={64--72},
year={1908},}

@ARTICLE{Jackson,
author={F. H. ~Jackson},
title={The basic gamme function and elliptic functions},
journal={proc. Roy. Soc.},
volume={A 76},
pages={127--144},
year={1905},}

@ARTICLE{ismail3,
 author={M. E. H.~Ismail},
 title={ The zeros of basic Bessel functions, the functions $J_{\nu+ax}$ and associated
orthogonal polynomials},
 journal={J. Math. Anal. Appl.},
 volume={86},
 year={1982},
 pages={11--19},
 }


@ARTICLE{IZ,
author={ M. E. H. Ismail and  Z. S. Mansour},
title={ $q$-Analogue of {Lidstone} expansion theorems, two-point {Taylor} expansions theorems and {Bernoulli} polynomials},
journal={ Analysis and Apllications.},
volume= { 17},
year={ 2019},
pages={853--895},}



@ARTICLE{Appell,
author={P. Appell},
title={Sur une classe de polyn$\hat{o}$mes},
journal={ Ann. Sci. Ec. Norm. Sup.},
volume={9},
pages={119--144},
year={1880},}

@BOOK{exton,
 author={H. Exton },
 title={$q$-{Hypergeometric} {Functions} and {Applications} },
 publisher={{New} {York}},
 edition={},
 address={},
 year={1983},}


@BOOK{Gasper,
 author={G.~Gasper and M.~Rahman },
 title={Basic {Hypergeometric} {Series}},
 publisher={Cambridge { University} Press},
 edition={second},
 address={Cambridge},
 year={2004},}

@Book{olver,
author={F. W. J. Olver },
title={{Asymptotics} and special functions},
publisher={Academic Press},
address={ New York.},
edition={ first},
year={ 1974},}


@Book{cramer,
author={D. Poole },
title={{Linear }{Algebra}. {A} {Modern} {Introduction}},
publisher={Cengage Learning.},
address={ },
edition={},
year={2014},}


@article{Alsalam1,
author={W. A. Al-Salam},
title={ $ q$-{Appell} polynomials},
journal={Ann. Mat. Pura Appl.},
volume= { 77},
pages={31--45},
year={ 1967},}

@article{Alsalam2,
author={W. A. Al-Salam},
title={{Some} fractional $q$-integrals and $q$-derviatives  },
journal={ Proc. Edinab. Math. Soc.},
volume= { 15},
pages={135--140},
year={ 1966/1967},}

@article{HN,
author={W. Hahn},
title={ Beitr$\ddot{a}$ge zur {Theorie} der {Heineschen}{ Rei-hen}},
journal={Math. Nachr.},
volume= {2},
pages={340--379},
year={ 1949},}

@article{Agarwal,
author={R. P. Agarwal},
title={ {Certain} fractional $ q$-integrals and $q$-derviatives},
journal={Proc.  Camb. Phil. Soc.},
volume= {66},
pages={365--370},
year={ 1969},}

@ARTICLE{two,
  AUTHOR =  " M. E. Keleshteri and N. I. Mahmoudov",
  TITLE =        "  A study on $q$-{Appell} polynomials from determinanatal point of view",
  JOURNAL =      " Appl. Math. Comput.",
  volume= {260},
pages={351--369},
  YEAR =   {2015},}

@Unpublished{marim,
  AUTHOR =       { Z. S.~ Mansour and  M.~ Al-Towalib},
  TITLE =        {The $q$-{Lidstone}  series involving $q$-{Bernoulli} and $q$-{Euler} polynomials generated by the third {Jackson} $q$-{Bessel} function},
  Note =         {Submitted},}

@Unpublished{sahar,
  AUTHOR =       { S.Z.H. Eweis and Z.S.I.~ Mansour },
  TITLE =        {{Generalized} $q$-{Bernoulli} polynomials generated by {Jackson} $q$-{Bessel} functions},
  Note =         {arxiv.org/abs/2201.10117},}

@book{cauchy,
author={L. Ahlfors},
title={{Complex} analysis. {An} introduction to the theory of analytic  functions of one complex variable},
publisher={  New York-Toronto-London:McGraw-Hill},
year={1953}},

@article{Frappier1,
author={C. Frappier},
title={ Representation formulas for entire functions of exponential type and generalized  {Bernoulli} polynomials},
journal={J. Austr. Math. Soc. Ser.},
volume= {64},
pages={307--316},
year={ 1998},}
@article{Frappier2,
author={C. Frappier},
title={ Generalized {Bernoulli} polynomials and series},
journal={ Bull. Austral. Math. Soc.},
volume= {61},
pages={289--304},
year={ 2000},}

@article{F3,
author={C. Frappier},
title={ A unified calculus Using the Generalized {Bernoulli} Polynomial },
journal={ J. Approx. Theory.},
volume= {109},
pages={279--313},
year={ 2001},}

}
@article{Sadj,
author={P. N. Sadjang},
title={ On a new q-analogue of {Appell} polynomials },
journal={ Math. CA.},
volume= {},
pages={1--17},
year={ 2018},}

